Conditional Generative Modeling via Learning the Latent Space

Although deep learning has achieved appealing results on several machine learning tasks, most of the models are deterministic at inference, limiting their application to single-modal settings. We propose a novel general-purpose framework for conditional generation in multimodal spaces, that uses latent variables to model generalizable learning patterns while minimizing a family of regression cost functions. At inference, the latent variables are optimized to find optimal solutions corresponding to multiple output modes. Compared to existing generative solutions, in multimodal spaces, our approach demonstrates faster and stable convergence, and can learn better representations for downstream tasks. Importantly, it provides a simple generic model that can beat highly engineered pipelines tailored using domain expertise on a variety of tasks, while generating diverse outputs. Our codes will be released.

==> figures/colorization_example_02.tex <==

\begin{figure}[h]
\centering
\captionsetup{size=small}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/1.png}
\end{subfigure} 
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/11.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/111.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/1111.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/11111.png}
\end{subfigure}

\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/2.png}
\end{subfigure} 
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/22.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/222.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/2222.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/22222.png}
\end{subfigure}

\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/3.png}
\end{subfigure} 
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/33.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/333.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/3333.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/color/itr/33333.png}
\end{subfigure}
\caption{The prediction quality increases as the $z$ traverse to an optimum position at the inference.} \label{fig:colorization_vis_02}
\end{figure}


==> figures/facade.tex <==
\begin{figure}
\captionsetup{size=small}

\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/gt1.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/gt2.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/gt3.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/gt4.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/gt5.png}
\end{subfigure}


\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/inp1.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/inp2.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/inp3.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/inp4.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/inp5.png}
\end{subfigure}


\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/predz1.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/predz2.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/predz3.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/predz4.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/facade/predz5.png}
\end{subfigure}

\caption{Image completion on Facade dataset with random masks.}  \label{fig:facde}
\end{figure}



==> figures/imgnet3.tex <==
\begin{figure}
\captionsetup{size=small}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out11g.png}
\end{subfigure}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out11.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out11c.jpg}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out11d.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out11a.png}
\end{subfigure} 
\hspace{5pt}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521g.png}
\end{subfigure}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521.png}
\end{subfigure}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521c.jpg}
\end{subfigure}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521d.png}
\end{subfigure}
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521a.png}
\end{subfigure}

\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out22g.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out22.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out22c.jpg}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out22d.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out22a.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553g.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553c.jpg}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553d.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553a.png}
\end{subfigure}

\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out27g.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out27.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out27c.jpg}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out27d.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out27a.png}
\end{subfigure}

\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out46g.png}
\caption{GT} \label{fig:4picsd}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out46.png}
\caption{Izuka} \label{fig:4picsd}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out46c.jpg}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out46d.png}
\end{subfigure} 
\begin{subfigure}{0.09\textwidth}
\includegraphics[width=\linewidth]{figures/imgnet/out46a.png}
\caption{Ours} \label{fig:4picsd}
\end{subfigure}
\caption{Qualitative comparison against the state of the art on Imagenet data. Our model generally produce more vibrant and balanced colors distributions.} \label{fig:colorimgnet}
\end{figure}

==> figures/inpainting_example_02.tex <==
% \begin{figure}
% \begin{tabular}{|c@{}c@{}c@{}c@{}c@{}c@{}|}
% {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_orig.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}}\\
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/023_orig.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/023_mask.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/023_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/023_comp.png}}\\
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/055_orig.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/055_mask.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/055_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}}\\
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/057_orig.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/057_mask.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/057_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}} \\
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/088_orig.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/088_mask.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/088_comp.png}} &
%  {\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}}\\
% \subfloat[GT]{\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/096_orig.png}} &
% \subfloat[Input]{\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/096_mask.png}} &
% \subfloat[C-Pyr]{\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/096_comp.png}} &
% \subfloat[Gan(s/c)]{\includegraphics[width =  0.4in]{figures/inpaint/paris/soart/006_comp.png}}
% \end{tabular}
% \caption{4 x 4}
% \end{figure}


==> figures/map.tex <==




==> figures/mnist_example_03.tex <==
% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[height=0.8in]{figures/mnist_train.PNG}
%         \caption{Training samples}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[height=0.8in]{figures/mnist_input.PNG}
%         \caption{Input}
%     \end{subfigure}
%     \caption{Market dashboard}
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[height=0.8in]{figures/mnist_train.PNG}
%         \caption{Market category lemonade}
%     \end{subfigure}
%     \caption{Market dashboard}
% \end{figure}

==> figures/related_work.tex <==
\section{Related work}

\textbf{Conditional Generative Modeling.}
Conditional generation involves learning a representation of a data distribution followed by conditioned sampling of the learnt distribution. With the success of \textit{VAEs} \citep{vaePaper} and \textit{GANs} \citep{ganPaper} in standard generative modeling tasks, their conditioned counterparts \citep{cVAE, cGAN} have dominated conditional generative tasks recently \citep{vitoria2020chromagan, zhang2016colorful, isola2017image, contextEncoder, harmonizing, bicycleGAN, cvaegan, disentangle_im2im, pennet} (add 3D spectral papers) with the latter performing significantly better at high dimensional distributions like natural images. A distinct feature of GANs is its mapping of points from a random noise distribution to the various modes of the output distribution. However, in the conditional case where an additional loss is incorporated to enforce the conditioning on the input, the significantly better performance of GANs is achieved at the expense of multimodality; the conditioning loss pushes the GAN to learn to mostly ignore its noise distribution. In fact, some works intentionally ignore the noise input in order to achieve more stable training \citep{isola2017image, contextEncoder, DeepMV, tempoGAN}. 

\textbf{Multimodality.} \textit{Conditional VAE-GANs} are one popular approach for generating multimodal outputs \citep{cvaegan, bicycleGAN} using the VAE's ability to enforce diversity through its latent variable representation and the GAN's ability to enforce output fidelity through its learnt discrimanator model. \textit{Mixture models} \citep{min_loss, multiGAN, mdn_color} that discretize the output space are another approach. Domain specific \textit{disentangled representations} \citep{disentangle_im2im, disentangle_multimodal} and explicit encoding of multiple modes as inputs \citep{iGAN, isola2017image} have also been successful in generating diverse outputs. \textit{Sampling-based loss} functions enforcing similarity at a distribution level \citep{harmonizing} have also been succesful in multimoal generative tasks. Further, the use of additional \textit{specialized reconstruction losses} (often using higher-level features extracted from the data distribution) and attention mechanisms also achieves multimodality through intricate model architectures in domain specific cases \citep{pennet, min_loss, vitoria2020chromagan, zhang2016colorful, iizuka2016let, inpainting_01, inpainting_02, inpainting_03, inpainting_nips, iizuka2016let}. 

We propose a simpler direction through our domain-independant energy function based approach that also focusses on learning representations capable of better supporting downstream tasks.

==> figures/stl.tex <==
\begin{figure}
\captionsetup{size=small}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521g.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521c.jpg}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521d.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out521a.png}
\end{subfigure}


\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553g.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553c.jpg}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553d.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out553a.png}
\end{subfigure}


\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out580g.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out580.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out580c.jpg}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out580d.png}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out580a.png}
\end{subfigure}


\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out615g.png}
\caption{GT} \label{fig:4picsd}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out615.png}
\caption{Izuka} \label{fig:4picsd}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out615c.jpg}
\caption{Chroma} \label{fig:4picsd}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out615d.png}
\caption{CIC} \label{fig:4picsd}
\end{subfigure}
\begin{subfigure}{0.1\textwidth}
\includegraphics[width=\linewidth]{figures/stl/out615a.png}
\caption{Ours} \label{fig:4picsd}
\end{subfigure}

\caption{Qualitative comparison against the state of the art on STL data. Our model generally produce more vibrant and balanced colors distributions.} \label{fig:colorstl}
\end{figure}
